Explaining Models: An Empirical Study of How Explanations Impact Fairness Judgment

Ensuring fairness of machine learning systems is a human-in-the-loop process. It relies on developers, users, and the general public to identify fairness problems and make improvements. To facilitate the process we need effective, unbiased, and user-friendly explanations that people can confidently rely on. Towards that end, we conducted an empirical study with four types of programmatically generated explanations to understand how they impact people's fairness judgments of ML systems. With an experiment involving more than 160 Mechanical Turk workers, we show that: 1) Certain explanations are considered inherently less fair, while others can enhance people's confidence in the fairness of the algorithm; 2) Different fairness problems--such as model-wide fairness issues versus case-specific fairness discrepancies--may be more effectively exposed through different styles of explanation; 3) Individual differences, including prior positions and judgment criteria of algorithmic fairness, impact how people react to different styles of explanation. We conclude with a discussion on providing personalized and adaptive explanations to support fairness judgments of ML systems.

==> documentBody/a-leftovers.tex <==
\section{LEFTOVERS}

\FIXME{VL: Jon and everyone else, see if you have more to say regarding the above. Feel free to edit or add}

\textbf{----------------VL: I think we seriously run out of space. Probably should exclude the content below}
\subsection{Lessons learned from explanation generation}
Different from Binns et al.~\cite{Binns2018a}, we developed programs to automatically generate these explanations. In this process, we uncovered a few statistical and design issues that may be useful to consider for future work to do automatic generation of these explanations. We briefly discuss 

\subsubsection{How to generate impact level in influence-based explanation}
\subsubsection{What's in the sensitivity of sensitivity-based explanation}
\subsubsection{When case-based explanation fail}








%\boldify{These systems have extremely poor published accuracy. We match it (around 67\%)}

After creating this system, we set out to understand its characteristics.
First, our raw data classifier had a test accuracy of 67.1\%, while the processed data classifier did slightly better at 67.6\%.
Note that these accuracies are low, but comparable to the findings of Equivant and ProPublica~\cite{NorthPointeValid, Larson2016}.
Additionally, we confirmed that the class labels in the data set were well balanced.
\FIXME{not included here, we are only using 5 features as toy data, but may mention the number in the method }

\boldify{In how many cases do the two classifiers differ in terms of prediction?}

The next question we set out to answer is: How different are the two classifiers in terms of predictions?  Of the 1056 test examples, there were 15 disagreements between the two classifiers

\FIXME{not included, we are de-emphasizing the processing techniques in the current framing}
\boldify{How many cases have NULL sensitivity explanations? what characterizes them?}

Some test examples would exhibit sensitivity to no features, which leads to what we consider a null sensitivity explanation.  
Of the 1056 test examples, this occurred 19 times with the raw data classifier, and 26 times with the processed data classifier.
However, the characterization of these examples is notable for several reasons.
First, all of the null sensitivity explanations are cases where the classifier is highly confident (Null cases: raw classifier confidence mean=90\% min=89\%, proc classifier confidence mean=92\% min=91\%).
Second, not all the highly confident cases have a null sensitivity explanation (Explained cases: raw classifier confidence mean=66\% max=89\%, proc classifier confidence mean=66\% max=87\%).


\boldify{How many cases are sensitive to the discriminatory features? What characterizes them?}

Sensitivity to the discriminatory features is of particular concern, since the goal of marginalizing out the effect of these features is to minimize their effect.
So how many examples exhibited this sensitivity? 
The raw data classifier showed this behavior 38 times, while the processed data classifier showed it only 3 times.
Again, the characterization of these examples is notable, since all of them lie \emph{on the decision boundary} --- the raw data classifier's confidence on examples which were sensitive to the discriminatory bit had an average of 52\% and a max of 54\%.
This effect was even stronger in the processed data classifier, with average and max confidence both at 50\%.


\FIXME{VL: will work on integrating to point 2 }

%\FIXME{JED: I am dubious of the claim that this has not been studied.  
%From an explanation perspective in the programming domain, the Whyline attacks exactly this issue: the output is a combination of both inputs AND some workflow to combine them.
%I think Lim intelligibility types would also point to similar difference?}

\boldify{How many exact FEATURE space matches are typical in a case based explanation?}

There is a tradeoff between having brief global descriptions and having meaningful local explanations.
This is because nearest neighbor search does not mean much if you have hundreds of exact matches due to tiny feature space, but global explanations grow as features*categories.
Given the feature space used in our study, we found the number of match counts distributed similarly between the 2 classifiers.
The combined distribution has mean=83$\pm$71, and a median of 65 (skewed left).
This indicates that while \emph{most} of the time, exact feature matches will be available, we must have a strategy for when they are not (5 instances have no exact feature space match, and 53 instances, or 5\% of the test data, had fewer than 5 matches).


\boldify{Of the exact matches found in a case based explanation, what \% of them also match LABEL?}

So now that we know how many exact matches one can expect in this problem, the next question is what \% of those feature matches also match the \emph{label} of the instance being explained.
This question is akin to asking if there are times when attempting to justify the prediction in this way will fail --- which Figure~\ref{figCaseMatchPercent} indicates is very possible.
\FIXME{stats requested are (1056 total test samples): \\
1. claim contradicted ($\leq 50\%$ match label)  =173 instances (16\% of the test data)\\
2. no claim justified (between $> 45\%$ and $< 55\%$ match label) =254 instances (24\% of the test data)\\
3. Correlation of match percent and confidence (df['match\_percent'].corr(df['confidence']))
=0.75761942076011424
}

\input{figure/caseMatchPercent}

\FIXME{VL: will work on integrating to point 3. I wonder if the figure is necessary. I probably just need some statistics to prove that case based can fail: 1)median of number of exact match , how often 0 matches, how often less than 5 matches; 2)how often equal or less than 50 percent matching label. Maybe, there is a point to make about the correlation between case based explanation and confidence---that can be a benefit of case-based explanation. is it hard to generate a correlation between confidence and the percentage matching label?? }

\boldify{Does any literature suggest that different explanations in different regions of feature space would perform better? Not sure, but we do!}

The results presented in this section indicate that different explanations may be better suited for different regions of feature space.
We have seen how case based explanations can fail to justify the intended example.
Similarly, we have seen how some examples are so clear cut that \emph{no} perturbation to them changes the prediction, while others are so unclear that \emph{any} perturbation changes the prediction.

\boldify{Active learning with confidence sampling: a possible motivation for oversampling region where the *output* (or explanation) is different.  There is an opportunity for us to recommend a sampling strategy here}

\FIXME{JED: Not sure where this idea goes, but we want it in the paper someplace, and I think it may follow from the above. perhaps we should argue that we are justifying the more difficult cases to justify?}



%We were particularly concerned with these issues since. Lee has shown that trust in algorithmic decisions is substantially lower than human ones~\cite{Lee2018}.
%Thus, one of our design goals was to make the explanations \emph{necessarily} sound by basing the explanation on the training data, the classifier's internal workings, or the classifier's behavior.

%Calders~\cite{Calders2013} and \v{Z}liobait{\.{e}} argue that these approaches can still lead to discrimination. 
%They define discrimination is present when, ``2 individuals that have the same characteristic relevant to the decision making and differ only in the sensitive attribute [and] the model results in different decisions.''
%Using small toy datasets to illustrate their argument, the authors lay out various ways in which bias can still creep in due to problems in sampling (biased sample, incomplete features, correlated features) and incorrect labeling (particularly a problem with subjective labeling).
%Most ML models assume that samples are independently identically distributed (IID), which could lead to poor performance if the initial sample is not representative of the population, or if the population changes over time.

%Some transformations (such as changing the discriminatory variable) are punished so heavily that they cannot happen.



%To manipulate the fairness of the classifier, we applied a preprocess intended to prevent discrimination in an automated fashion (similar to~\cite{Calmon2017}).

%By measuring both ``actual''  fairness and human perception of fairness in the classifier's decisions, we will be able to determine how they are correlated (RQ1).
%Depending on the existence and quality of this correlation, it will shed light on the usefulness of treating humans' perception of fairness as a ground truth measure.

%\boldify{At a high level, what is the problem?}

%We assessed human perceptions of fairness in ML classifiers as we manipulated two factors: 
%(1) the amount of \emph{measurable} fairness present in classifiers and (2) different kinds of explanations of the classifier's decision process.
%\FIXME{VL comment: I have been thinking about our setup. In fact we manipulated two ``fairness issues'', one is the overall classifier, the other is the region---it is less fair to rely on the system for boundary cases. What we found is a significant effect between global v.s. local that interacts with ``impacted'', showing that local explanation is better at exposing fairness issue caused by different cases/regions}

%\boldify{ML is statistical, but can still discriminate, which is why we need to debias}




%\boldify{Now that we have established the need for debiasing, how does ours work?}

%In our work, we chose to use a preprocessor that transforms the data, though we do not use a new representation space~\cite{Calmon2017}.
%This technique does this by marginalizing out the effect of the discriminatory variable(s) by attaching penalties to changing features in the training data.
%The result of applying the preprocessor is a new dataset which is ``fairer'' while also limiting local deformations because the penalties rise with the magnitude of the feature change (e.g. changing a persons age from 5 to 60 will result in a higher penalty than changing their age from 5 to 8).


%\boldify{Why can't we just axe the feature?}

%Perhaps all this sounds complicated, and the reader is wondering, ``Why can't we just drop the discriminatory feature(s)?''
%Well, Calders and \v{Z}liobait{\.{e}} indicate that this ``does not help if some other attributes are correlated with the sensitive attribute''~\cite{Calders2013}.
%Further, once that feature is removed, discovering any correlations with other features becomes impossible.
%Another strategy to consider is dropping the discriminatory feature and all features which are correlated with it.
%However, some features carry ``objective information'' about the label.
%To illustrate this, they present the case of the \emph{postal code}, which is both ``related to ethnicity, but also carries information about real estate prices''~\cite{Calders2013}.


% \FIXME{VL comment: Maybe, we should have a separate use case section in methodology to discuss COMPA. A little distracting here. will come back and decide}
%\boldify{How will we surface whether the classifier is fair or not? Explanation!}

%In order to reveal the ``fairness'' of the classifier, we used explanations of its individual decisions.
%To determine the structure and content of our explanations, we consulted the literature.
%Kulesza et al. presented results from varying explanations along the soundness/completeness axes~\cite{Kulesza2013}.
%They found that the best mental models arose from explanations with both high completeness and high soundness.
%Thus, one of our design goals was to make the explanations \emph{necessarily} sound by basing the explanation on the training data, the classifier's internal workings, or the classifier's behavior.





%Recently, a group of journalists at ProPublica, led by Larson, provided a deep statistical analysis on the prediction accuracy of the COMPAS algorithm~\cite{Larson2016, ProPublicaData}.
%Their methodology was to collect a new data sample and evaluate the existing model's accuracy on it.
%They found several troubling issues:
%First, the classifier has low accuracy (ProPublica found 63.6\%, the application developers found 68\%, both of which are quite low). 
%Second, while the \emph{accuracy} is similar across racial features (62.5\% vs 62.3\%), the confusion matrix shows that, in terms of their risk to recidivate, black defendants are frequently overestimated, while white defendants are often underestimated.


%This software's creators performed a lengthy analysis of the validity of its predictions, and found ``that it preformed [sic] equally well for African American and White men at predicting the arrest outcomes''~\cite{NorthPointeValid}.




%In response to this analysis, Northpointe refuted ProPublica's claims~\cite{NorthPointeResponse}, for which ProPublica had its own response~\cite{PropublicaResponse}.
%Thus, it potentially remains an open question on whether or not these classifiers are ``fair'' in the abstract sense



%To manipulate the fairness of the classifier, we applied a preprocess intended to prevent discrimination in an automated fashion (similar to~\cite{Calmon2017}).
%There are several different definitions of fairness, for example:
%\quotateInset{...discrimination is considered to be present if for two individuals that have the same characteristic relevant to the decision making and differ only in the sensitive attribute (e.g., gender or race) a model results in different decisions~\cite{Calders2013}.}
%By measuring both ``actual''  fairness and human perception of fairness in the classifier's decisions, we will be able to determine how they are correlated (RQ1).
%Depending on the existence and quality of this correlation, it will shed light on the usefulness of treating humans' perception of fairness as a ground truth measure.
%\FIXME{VL comment: need layman terms on what pre-processing did here. Instead of framing it as ``correlate'', I would phrase it as we manipulated ``fairness issue'' by having the two different data conditions, and see which type of explanation is better at exposing it. Will work on it if you agree}


%\boldify{Describe experimental factor 2: Explanation}

%The other factor manipulated is the type of explanation provided to the participant.
%Prior work has examined various types of explanation and how they impact the quality of the mental model the user has about the classifier~\cite{Kulesza2013}.
%Similarly, prior work has examined fairness of classifiers~\cite{FIXME, Grgic-Hlaca2018, Binns2018a}.
%However, to the best of our knowledge, no one has investigated human perception of a classifier's fairness using programmatically generated explanations.
%\FIXME{VL comment: need a brief discussion on the concept of ``global versus local'' explanation, as well as process versus data based explanation. One of the interesting qual results I found is that people found sensitivity and influence told them more about *how* the algorithm works, while for case and demographic they commented more on the data...  will decide if putting RQ before or after background.}


%Before choosing individuals to present to participants, we first removed all the individuals with no feature sensitivities from either classifier (26 instances).
%This was done to ensure that each explanation shown would be well defined for the participant.
%From this pool, individuals we selected came from two groups, the first of which was composed of individuals for which the raw classifier was sensitive to the discriminatory variable (the ``Disparately Impacted'' group, 23 instances).
%The second group comprised individuals for whom this was not the case \emph{and} the two classifiers agreed on prediction (the ``Non Impacted'' group, 992 instances).
%Next, we filtered each sample group for unique individuals, leaving 8 in the Disparately Impacted group.
%Last, a random subsample of the Non Impacted group was selected, chosen to be twice the size of the final Disparately Impacted group (16 instances). 
%Since the second group was so much larger than the first group, we showed four Non Impacted individuals and two Disparately Impacted individuals to each participant, in a random order.






%\boldify{Set up the overall goals and how we will break down the section (1. classifier config 2. generating explanations 3. Debiasing 4. Survey Evaluation }

%Our goals were to measure the participants perceptions of the fairness of the classifier as we manipulated two factors: the type of explanation presented and the underlying fairness of the classifier.
%Before delving into these two subjects, we first discuss the configuration of the classifier and data set, before concluding with a discussion of the survey methodology used to test our approach.

%\subsection{Classifier Configuration and Data}

%\boldify{Ultimately, what we built is a wrapper around sklearn's linear classifier }

%First, the classifier we used is sklearn's\footnote{FIXME sklearn link. Mention class balance was checked and passed} logistic regression.
%Other options would have worked just as well, though it may impact the possible explanation types under this framework.
%Using a simple linear model is ecologically valid since, in practice, many decision support settings prefer interpretable models, and even sacrifice significant accuracy to improve interpretability and maintainability~\cite{Veale2018}.

%\boldify{A key thing for the reader to understand is how we manage feature/category names}

%We dummy coded the data prior to fitting the classifier, meaning that all categorical features are transformed into binary indicator variables.
%As a result, the feature names in our data frame are of the form \feature{<feature\_name>\_<category\_name>}, e.g. \feature{age\_30-39}
%These data frame column titles are used in the explanations with little processing.
%Further, the binary indicator variable construction allows for easy counterfactual generation, for example, we can simply move the bit from \feature{age\_30-39} to \feature{age\_40-49} to make an individual older.

%\boldify{So we have the big picture, but theres an important wrinkle: dropping columns!}

%One small detail that remains is to consider that logistic regression implicitly compares the feature vectors with one where all features are 0.
%Thus, the reference object becomes unclear if both sides of a dichotomous feature are present in the data frame.
%The same argument holds for categorical data and having all categories present in the data frame.
%The solution is to drop one category for all features, and remember what was removed.
%For our implementation, we used the median category where possible, and random selection otherwise.
%This allows for an interpretable reference object, though it does complicate generating some explanations\footnote{Consider a feature with $N$ categories.
%If we drop category $1$, then in order to determine if a sample has a feature value in category $1$, we must test for the absence of the other $N-1$ features.}.


%\subsection{Debiasing}
%\boldify{So what was the data we actually put in the data frame?}
%We chose to use the COMPAS data set because it is relatable to regular people, which lends itself to evaluation of explanations and fairness.
%Further, it is a commonly used data set in the study of fairness, with fine grained study about the fairness of using various types of data it contains~\cite{Grgic-Hlaca2018}.


%One of the advantages of using textual-only explanations is to control for differences in both representation and presentation.
%Visual explanations often use combinations of text, graphs, or other imagery to communicate information about the decision process.
%\FIXME{JED: Here we can use citations from Binns page 4, column 2.  Citations are 18, 62.  with the ``imagery'' part I meant saliency maps, which the vision community heavily uses for explanatory purposes.}


%The questions we chose to ask were based on Binns et al.~\cite{Binns2018a}, but we removed some questions to shorten the tasks.
%We added some additional questions based on [The XAI TA2 measuring trust report, really no idea if/how we can cite this]
%\FIXME{JED: Can we cite XAI TA2 reports.
%The questions we removed from the binns work were essentially all well studied by others (e.g. ``factors considered were fair'' was much better studied by \cite{Grgic-Hlaca2018}. 
%The questions we added were largely derived from the Cahour-Fourzy scale (which they cite) if we cannot figure out a way to point to the XAI TA2 report}
%\FIXME{VL comment: we don't need this figure. we don't use all questions. i will work on description)}





% \subsubsection{Prediction outcome} A couple of participants commented that the binary prediction itself is problematic and unfair, e.g., ``\textit{The machine should have produced a more refined risk assessment. [For example] in percentages.}'' (P176).

% \FIXME{JED: this should be cut, mostly because the ecologically valid approach does exactly this and we simplified it away.  I do not want this can of worms opened}





% \subsubsection{De-biasing by data processing}

% We divided up our features into three sets, $D, X,$ and $Y$, where $D$ is the set of discriminatory features, $X$ is the set of ``fair'' features, and $Y$ is the predicted variable (similar to~\cite{Calmon2017}).
% In this case, the prediction ($Y$) is whether or not this individual will reoffend.
% As for the inputs, $D$ contained only \feature{race}, while $X$ containing \feature{age}, \feature{charge}, \feature{priors}, and \feature{juvenile priors}.

% \FIXME{VL: this sub-section on processing is not good. will come back after working on literature review}






\boldify{Why model/explain for real? debugging}

Prior work that assesses human perception of fairness of ML decision processes used a wizard of oz methodology to generate explanations~\cite{Binns2018a}, while we would like to use real classifiers and their output.
This will allow us to gain insight on what participants attribute the \emph{source} of bias to be (RQ4).
This is important from a debugging perspective because it is akin to fault localization.

\boldify{Why model/explain for real? tech acceptance}

It is also important from a technology acceptance point of view;  if participants blame the data or the societal phenomenon it was sampled from, then preprocessing seems like a suitable fix.
However, if participants blame the classifier \emph{itself}, then perhaps understanding and improving alignment between the processes used by human and machine may be a more appropriate fix (RQ5).

\boldify{Some stuff about Calmon's paper}
They also present a measure by which we can claim a classifier is free of discrimination: given a predicted label, no classifier should be able to do better than random guessing at the discriminatory features (i.e. given a prediction of a convict reoffending, we should not be able to predict the race of an individual).



------------------------------------------


\FIXME{\color{blue}The subsequent paragraph on Binns seems to fit best where we are discussing choosing the data set and how well studied this is from a fairness perspective?\\}

Binns et al.~\cite{Binns2018b} examined the study of fairness in machine learning with a philosophical lens.
He describes some of the troublesome issues of the study of fairness, such the extent to which inference should be based on an individual's group memberships vs the choices they have made.

\FIXME{\color{blue}The subsequent paragraph on Woodruff seems to fit best where we discuss the myriad of studies on fairness (this one strictly qualitative) ?\\}

Woodruff et al.~\cite{Woodruff2018} engaged in a discussion with members of traditionally marginalized groups to discuss their experiences with algorithmic discrimination.
They found a wide variety of attitudes about the scope and source of such discrimination, as well as how to remedy it.

\FIXME{\color{blue}The subsequent paragraph on Conway seems to fit best where we are framing the design goals for explanation? Also needs to say what they found in their study\\}

Conway et al.~\cite{Conway2016} studied human-machine trust by manipulating the cues tied to an outcome in a traffic control system.
The system had several algorithms it could use in combination to control traffic, some of which were tied to a reductions, others were not.
Participants had to disentangle which algorithms were trustworthy.

\FIXME{\color{blue}The subsequent paragraph on Keren seems to fit best where we are framing the design goals for explanation?\\}

Keren et al.~\cite{Keren2007} presented experiments investigating how message framing impacts trust.
They varied whether the message was framed negatively (e.g. meat which is 25\% fat) or positively (e.g. meat which is 75\% lean), and found that people tend to \emph{trust} the negative framing, but \emph{choose} the positive.
This leads to what they term the \emph{trust-choice incompatibility}.

\FIXME{\color{blue}The subsequent paragraph on Teigen seems to fit best where we are framing the design goals for explanation?\\}

Teigen et al.~\cite{Teigen2009} also studied framing, examining perception of authoritative predictions that turned out incorrect.
They found that pessimistic statements were perceived better.
This means that they recommend a negative framing for choices that perform \emph{worse} than expected, and a positive framing for choices that perform \emph{better}.


\FIXME{JED: This citation seems like one we should use, but I dont really understand it well.~\cite{Pedreschi2008}}



The term ``disparate impact'' stems from US law, particularly in housing and labor, and refers to practices which adversely affect people of one protected characteristic more than another~\cite{FIXME}.
The test to determine its presence is referred to as the ``80\% rule''~\cite{FIXME some court decision}, intended to ensure balance in the selection among groups formed by protected characteristic.
In fact, this rule is the inspiration for one of the statistical formulas used in data preprocessing\footnote{It is formula 2, and it essentially states that the probability of outcomes given the discriminatory feature $d \in D$ are similar for all groups in $D$.
Note that this is more tied to group fairness than individual fairness both in terms of technical approaches~\cite{Dwork2012, Feldman2015} and policy designed to investigate and mitigate disparate impact~\cite{Barocas2016, Pickerill2009}.
}~\cite{Calmon2017}.

Disparate impact need not be intentional  --- then it is disparate treatment.
Calders defines this as ``When such rules or practices explicitly treat one person less favorably on a forbidden ground than another is, has been or would be treated in a comparable situation''~\cite{Calders2013}.
This definition indicates the importance of \emph{comparable situation} in disparate impact/treatment.
Grgic-Hlaca emphasize the future results more, whether the practice, ``may increase disparity in outcomes'' or ``would result in protected group members receiving disadvantageous treatment''~\cite{Grgic-Hlaca2018}.




==> figure/caseMatchCount.tex <==
\begin{figure}
	\centering
    \includegraphics[width=\columnwidth]{assets/caseMatchCount}
	\caption{FIXME case based explanation match count histogram.}
	\Description{FIXME}
    \FIXME{What I am trying to show here is that the number of ``cases'' available will vary widely, in this case, from a few hundred exact matches to 0 exact matches.
    Therefore, 0 matches is an eventuality we must prepare for (and we do so, falling back on nearest neighbor search).
    }
	\label{figCaseMatchCount}
    %\vspace{-10pt} % this line can be used to eat whitespace before/after the figure if needed
\end{figure}



==> figure/caseMatchPercent.tex <==
\begin{figure}
	\centering
    \includegraphics[width=\columnwidth]{assets/caseMatchPercent}
	\caption{FIXME case based explanation match percent histogram.
    }
    \Description{FIXME}
    \FIXME{
    What I am trying to show here is that sometimes ``justification'' fails when we try to use case based reasoning.\\
    I.e. Classifier think this person will reoffend because... 0 of the 9 ppl in training data who are identical reoffended?\\
    Huh????  \\
    If we keep this one, I think we should shrink the Y range to highlight the amount of probability mass below X =.5 (the region where the justification *fails*).
    Notably, in these cases, global considerations for the placement of the decision boundary were more important than the local ones (correctly classifying training examples in the region), so this region is being consistently misclassified.
    The problem with shrinking it is that it fails to highlight how much probability mass resides around 50\% (i.e. case based justification provides no evidence for any label)
    }
	\label{figCaseMatchPercent}
    %\vspace{-10pt} % this line can be used to eat whitespace before/after the figure if needed
\end{figure}

==> figure/confidenceBoxPlot.tex <==
\begin{figure}
	\centering
    \includegraphics[width=\columnwidth]{assets/confidenceBoxPlot}
	\caption{FIXME boxplot of confidence of samples with and without a sensitivity-based explanation.
    }
    \Description{FIXME}
    \FIXME{
    What I'm trying to communicate here is that the confidence distributions of the samples with NULL sensitivity explanation are markedly different from the rest of the samples.
    However, the distributions are not necessarily disjoint (in the raw data case), so confidence alone is an insufficient predictor of when this type of explanation will be well defined, if we were trying to build an ``automatic explanation style chooser.''
    }
	\label{figConfidenceBoxPlot}
    %\vspace{-10pt} % this line can be used to eat whitespace before/after the figure if needed
\end{figure}

==> figure/geometric.tex <==
\begin{figure}
	\centering
    \includegraphics[width=.8\columnwidth]{assets/geometric.pdf}
	\caption{Our explanations are based on 2 main parts, the decision boundary (solid green line), the training data (set of blue X and red O).
    To explain the decision for an input (numbered purple squares), then explaining via:
    1) Input-Influence requires \emph{only} the decision boundary,
    2) Demographics requires the training data and its distribution with respect to the decision boundary,
    3) Case involves nearest neighbor search around the input, and
    4) Sensitivity relies on projecting axis aligned lines from the input to the decision boundary (dashed black lines).
    }
    \Description{FIXME}
	\label{figGeometric}
    \FIXME{JED: My caption is verbose and needs to be audited together with the text for duplication}
    %\vspace{-10pt} % this line can be used to eat whitespace before/after the figure if needed
\end{figure}

==> figure/scenario.tex <==
\begin{figure}
    \footnotesize
    \flushleft
    \fbox{\color{black}%
			\parbox{.97\linewidth}{
            \textbf{Scenario} a machine learning software has been introduced to help a judge decide whether a person who has been charged with a crime should be given bail, and if so, its amount.
A critical consideration in a bail decision is the defendant's ``risk'', including the probability that the individual will commit another crime (re-offend).
To support the risk assessment, the machine learning software makes a prediction on whether an individual is likely to reoffend based on historical data collected about a few thousand other people charged with crimes.
The output of the software is a prediction of whether or not the individual is likely to reoffend.
			} 
           }
	\caption{Scenario shown to each participant. 
    We also summarized the data available, both features and categories.
    }
    \Description{FIXME}
	\label{figScenario}
    \vspace{-10pt} % this line can be used to eat whitespace before/after the figure if needed
\end{figure}
